Prior-agnostic Multi-scale Contrastive Text-Audio Pre-training for Parallelized TTS Frontend Modeling

Over the past decade, a series of unflagging efforts have been dedicated to developing highly expressive and controllable text-to-speech (TTS) systems. In general, the holistic TTS comprises two interconnected components: the frontend module and the backend module. The frontend excels in capturing linguistic representations from the raw text input, while the backend module converts linguistic cues to speech. The research community has shown growing interest in the study of the frontend component, recognizing its pivotal role in text-to-speech systems, including Text Normalization (TN), Prosody Boundary Prediction (PBP), and Polyphone Disambiguation (PD). Nonetheless, the limitations posed by insufficient annotated textual data and the reliance on homogeneous text signals significantly undermine the effectiveness of its supervised learning. To evade this obstacle, a novel two-stage TTS frontend prediction pipeline, named TAP-FM, is proposed in this paper. Specifically, during the first learning phase, we present a Multi-scale Contrastive Text-audio Pre-training protocol (MC-TAP), which hammers at acquiring richer insights via multi-granularity contrastive pre-training in an unsupervised manner. Instead of mining homogeneous features in prior pre-training approaches, our framework demonstrates the ability to delve deep into both global and local text-audio semantic and acoustic representations. Furthermore, a parallelized TTS frontend model is delicately devised to execute TN, PD, and PBP prediction tasks, respectively in the second stage. Finally, extensive experiments illustrate the superiority of our proposed method, achieving state-of-the-art performance.

==> sections/4_problem.tex <==
\section{Problem Statement}
% % 本节以一些基本符号来定义我们要解决的问题。
% % 目前我们在TTS前端中每个子任务各有一个规模相对较小纯文本的精标数据集，TN的数据集是Dtn，PB的数据集是Dpb，PD的数据集是Dpd，另外还有一个数据规模很大的成对存在的文本-音频数据集Dpre,其中文本表示为Tpre，对应的音频表示为Apre。
This section defines the problem we are going to solve by using basic symbols.
Currently, each subtask in our TTS frontend has a relatively small annotated dataset consisting of pure texts. The dataset for TN is $\Set{T}_{TN}$, for PBP is $\Set{T}_{PBP}$, for PD is $\Set{T}_{PD}$, and there is also a large-scale paired text-audio dataset $\Set{D}_{pre}$, where the text is represented as $\Set{T}_{pre}$ and the corresponding audio is represented as $\Set{A}_{pre}$.

% 问题分为两个阶段
% stage 1：在Dpre上使用文本-音频对比预训练的方式来训练一个文本编码器，让他在具有语义特征的同时学习到音频特征，定义为
% PTextEncoder = P(TextEncoder，WavEncoder,Tpre,Apre)

% stage 2：使用预训练好的TextEncoder，给定输入文本t_task,task属于{TN，PB，PD}，目标是学习一个模型，可以输出对应任务的预测结果\hat{y}_{task}
The \textbf{problem} is divided into two stages.


\textbf{Stage 1}: Train a text encoder on $D_{pre}$ using text-audio contrastive pretraining to learn both semantic and audio features. This is defined as:
\begin{equation}
    \begin{split}
        \mathrm{PTextEncoder} = P(\mathrm{TextEncoder}, \\ \mathrm{WavEncoder},
        \Set{T}_{pre},\Set{A}_{pre}).
    \end{split}
\end{equation}


\textbf{Stage 2}: Using the $\mathrm{PTextEncoder}$, given input text $t_{task}$, where $task \in \{TN, PBP, PD\}$, the objective is to learn a model that can output the predicted result $\hat{y}_{task}$ for the corresponding task. This is defined as:
\begin{equation}
    \hat{y}_{task} = f(\mathrm{PTextEncoder},t_{task})
\end{equation}
% 在推理的时候$task$可以是一个，也可以是多个
When reasoning, $task$ can be one or multiple.


